Show, Don't Tell: Learning Reward Machines from Demonstrations for Reinforcement Learning-Based Cardiac Pacemaker Synthesis

An (artificial cardiac) pacemaker is an implantable electronic device that sends electrical impulses to the heart to regulate the heartbeat. As the number of pacemaker users continues to rise, so does the demand for features with additional sensors, adaptability, and improved battery performance. Reinforcement learning (RL) has recently been proposed as a performant algorithm for creative design space exploration, adaptation, and statistical verification of cardiac pacemakers. The design of correct reward functions, expressed as a reward machine, is a key programming activity in this process. In 2007, Boston Scientific published a detailed description of their pacemaker specifications. This document has since formed the basis for several formal characterizations of pacemaker specifications using real-time automata and logic. However, because these translations are done manually, they are challenging to verify. Moreover, capturing requirements in automata or logic is notoriously difficult. We posit that it is significantly easier for domain experts, such as electrophysiologists, to observe and identify abnormalities in electrocardiograms that correspond to patient-pacemaker interactions. Therefore, we explore the possibility of learning correctness specifications from such labeled demonstrations in the form of a reward machine and training an RL agent to synthesize a cardiac pacemaker based on the resulting reward machine. We leverage advances in machine learning to extract signals from labeled demonstrations as reward machines using recurrent neural networks and transformer architectures. These reward machines are then used to design a simple pacemaker with RL. Finally, we validate the resulting pacemaker using properties extracted from the Boston Scientific document.

==> sequence_classifiers.tex <==
\subsection{Sequence Classifiers}\label{sequence-classifier}

In this work, we investigate two DL architectures as reward machines: bi-directional LSTMs and transformer networks.

\subsubsection{Bi-Directional LSTMs}

LSTMs \cite{lstm} are a type of recurrent neural network (RNN) that can hold pattern--information in their cell states through the succession of large sequences. We start this section by providing an overview of RNNs, followed by an overview of the specific mechanisms of LSTMs.

Given an input sequence $\{ x_1 , x_2, \ldots, x_t\}$, we want to obtain a sequence of outputs $\{y_1 , y_2, \ldots, y_t\}$. Assuming a one-layer RNN, to compute an output $y_t$ for an input $x_t$, we need the activation value for the hidden layer $h_t$. 
This value can be computed as:
\begin{align}
    h_t &= g(U h_{t-1} + W x_t) \\
    y_t &= f(V h_t) \label{eq:output}
\end{align}

\noindent Where $U$, $W$ and $V$ are learnable weight matrices, and $g$ corresponds to a non-linear activation function. As we can observe, hidden states and each time step $t$ depend on hidden states at previous time steps $t-1$. This operation defines the recurrence that encodes the sequential information. Finally, output $y_t$ is computed using function $f$. Typically for classification tasks, $f$ consists of softmax computation that provides a probability distribution over the possible output classes. While the above formulation deals with a single layer, more RNN layers can be stacked by using
the entire sequence of outputs from one RNN layer as the input sequence to another one.

LSTMs improve on the information retention capabilities of RNNs by introducing mechanisms that learn weighted importance of previous timesteps. This is done using a ``forget'' gate which assigns values between $0$ or $1$ to previous cell states. A weight of $0$ results in the current cell discarding older information, and a weight of $1$ keeps entire state in memory. 

Given inputs $ \{ x_1 , x_2, \ldots, x_t\}$ with respective cell states $ \{ c_1 , c_2 , \ldots, c_t\}$, an LSTM produces hidden states $ \{ h_1 , h_2 , \ldots, h_t\}$ using the computation described below. 
\begin{align}
    f_t &= \sigma (U_f h_{t-1} + W_f x_t) \\
    k_t &= c_{t-1} \odot f_t
\end{align}

\noindent Here, $U_f , W_f$ are the learnable weight matrices associated with the forget gate, $f_t$ is the output from a sigmoid function that weights previous context $c_{t-1}$. In the next step, we calculate current information $g_t$ using learnable weights matrices $U_g, W_g$ as:
\begin{align}
    g_t = \mathtt{tanh}(U_g h_{t-1} + W_g x_t)
\end{align}

Then, we use an add gate $i_t$ to decide how much of the current context $g_t$ should be considered going forward:
\begin{align}
    i_t &= \sigma (U_i h_{t-1} + W_i x_t)\\
    j_t &= i_t \odot g_t 
\end{align}

Lastly, we calculate the current cell state $c_t$ and hidden state $h_t$ as follows: 
\begin{align}
    c_t &= j_t + k_t\\
    o_t &= \sigma (U_o h_{t-1} + W_o x_t)\\
    h_t &= o_t \odot \mathtt{tanh}(c_t)
\end{align}

The output gate $o_t$ weighs how much of $c_t$ should be available as information for future states. $U_i , W_i$ and $U_o, W_o$ are the learnable weight matrices associated with the \textit{add gate} and \textit{output gate}, respectively. As in the case of vanilla RNNs, the hidden state $h_t$ is then either passed to another LSTM layer, or passed through a softmax layer (see equation \ref{eq:output}) to obtain the final output $y_t$.  \footnote{Our notation are based on Jurafsky and Martin~\cite{slp}.} 

Bi-directional LSTMs differ from regular LSTMs as they consider the sequence in the regular and reversed orders. This allows the model to consider information occurring at the beginning and end of the sequence simultaneously. The computation will remain the same, but the inputs and outputs will be concatenated in the following manner: 
\begin{align}
    \{ h_{1} , h_{2} \dots h_{t} \} \xrightarrow{} \{h_1 : h_{t} , h_2 : h_{t-1} \dots h_t : h_{1} \}\\
    \{ x_{1} , x_{2} \dots x_{t} \} \xrightarrow{} \{x_1 : x_{t} , x_2 : x_{t-1} \dots x_t : x_{1} \} 
\end{align}

As all neural networks, bi-directional LSTMs can be learned via gradient-based methods using a differentiable loss function. In the case of classification tasks, this loss is typically the cross-entropy loss. 


\subsubsection{Transformer Networks}

Transformer networks \cite{transformers} eschew recurrence information and use attention mechanisms to gather sequential information. 
Transformers can attend to arbitrary pairs of actions in pacemaker traces, potentially allowing them to better differentiate between correct and incorrect patterns.

In this section, we describe single-layer and single-head transformer self-attention for a input sequence $ \{ x_1 , x_2 , x_3 \dots x_t\}$ with respective hidden activations $ \{ h_1 , h_2 , h_3 \dots h_t\}$. 
To calculate self-attention at position $x_i$ with respect to all other positions $x_j$, we initialize three weight matrices as follows: 
\begin{align}
    W^Q &\xrightarrow{} \text{Weight matrix of } x_i \text{ (query)}\\
    W^K &\xrightarrow{} \text{Weight matrix of } x_j \text{ (key)}\\
    W^V &\xrightarrow{} \text{Weight matrix of } \texttt{score}(x_i , x_j) \text{ (value)}
\end{align}

 
When we focus on the self-attention of $x_i$, we consider $x_i$ to be the ``query'', and all other $x_j$ to be the ``key''. In order to capture the importance of a particular pair, we consider it to be its ``value''. Using this, we can calculate the \textit{query}, \textit{key} and \textit{value} vectors as follows: 
\begin{align}
    q_i &= x_i \cdot W^Q\\
    k_j &= x_j \cdot W^K\\
    v_j &= x_j \cdot W^V\\
    h_{ij} &= \mathtt{softmax}(\frac{q_i \cdot k_j}{\sqrt{d_k}}) v_j
\end{align}

These operations can be parallelized for all $x_i$ by horizontally stacking $q_i$, $k_i$, $v_i$ for each $x_i$. These stacked vectors become matrices and are denoted by $Q$, $K$ and $V$, respectively. The operations in the previous equations can thus be calculated all at once as: 
\begin{align}
    H &= \mathtt{softmax}(\frac{QK}{\sqrt{d_k}})V
\end{align}

Here, the value $\sqrt{d_k}$ serves to scale the dot product of $Q \cdot K$. Since the derivative of a softmax is close to $0$ for large products, the scaling factor pushes the value down to improve convergence and allow for quicker training.      

As in the case of LSTMs, hidden activations $ \{ h_1 , h_2 , h_3 \dots h_t\}$ can be passed to other self-attention layers, or to a softmax layer (see equation~\ref{eq:output}) to obtain a probability distribution over the possible output classes. In practice, transformer networks utilize multiple self-attention layers. Over-parametrized transformers trained over massive amounts of data and have been shown to be very good at extracting sequence information such as hierarchy and syntax.

As all neural networks, transformers can be learned via gradient-based methods using a differentiable loss function. A possible limitation of using transformers is that they require large amounts of data to learn. We try to offset this problem by choosing shallower transformers with fewer learnable weights. 
